Dependency Decomposition and a Reject Option for Explainable Models

Deploying machine learning models in safety-related do-mains (e.g. autonomous driving, medical diagnosis) demands for approaches that are explainable, robust against adversarial attacks and aware of the model uncertainty. Recent deep learning models perform extremely well in various inference tasks, but the black-box nature of these approaches leads to a weakness regarding the three requirements mentioned above. Recent advances offer methods to visualize features, describe attribution of the input (e.g.heatmaps), provide textual explanations or reduce dimensionality. However,are explanations for classification tasks dependent or are they independent of each other? For in-stance, is the shape of an object dependent on the color? What is the effect of using the predicted class for generating explanations and vice versa? In the context of explainable deep learning models, we present the first analysis of dependencies regarding the probability distribution over the desired image classification outputs and the explaining variables (e.g. attributes, texts, heatmaps). Therefore, we perform an Explanation Dependency Decomposition (EDD). We analyze the implications of the different dependencies and propose two ways of generating the explanation. Finally, we use the explanation to verify (accept or reject) the prediction

==> figures/gtsrb.tex <==
\begin{figure}[!ht]
	\centering
	%\figsp
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/00} 
		\vspace{4ex}
	\end{subfigure}%% 
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/01} 
		\vspace{4ex}
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/02} 
		\vspace{4ex}
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/03}
		\vspace{4ex} 
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/04} 
		\vspace{4ex}
	\end{subfigure}%% 
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/05} 
		\vspace{4ex}
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/06} 
		\vspace{4ex}
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/07}
		\vspace{4ex} 
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/08} 
		\vspace{4ex}
	\end{subfigure}%% 
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/09} 
		\vspace{4ex}
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/10} 
		\vspace{4ex}
	\end{subfigure} 
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/11} 
		\vspace{4ex}
	\end{subfigure}%% 
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/12} 
		\vspace{4ex}
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/13} 
		\vspace{4ex}
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/14}
		\vspace{4ex} 
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/15} 
		\vspace{4ex}
	\end{subfigure}%% 
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/16} 
		\vspace{4ex}
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/17} 
		\vspace{4ex}
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/18}
		\vspace{4ex} 
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/19} 
		\vspace{4ex}
	\end{subfigure}%% 
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/20} 
		\vspace{4ex}
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/21} 
		\vspace{4ex}
	\end{subfigure} 
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/22} 
		\vspace{4ex}
	\end{subfigure}%% 
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/23} 
		\vspace{4ex}
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/24} 
		\vspace{4ex}
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/25}
		\vspace{4ex} 
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/26} 
		\vspace{4ex}
	\end{subfigure}%% 
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/27} 
		\vspace{4ex}
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/28} 
		\vspace{4ex}
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/29}
		\vspace{4ex} 
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/30} 
		\vspace{4ex}
	\end{subfigure}%% 
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/31} 
		\vspace{4ex}
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/32} 
		\vspace{4ex}
	\end{subfigure} 
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/33} 
		\vspace{4ex}
	\end{subfigure}%% 
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/34} 
		\vspace{4ex}
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/35} 
		\vspace{4ex}
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/36}
		\vspace{4ex} 
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/37} 
		\vspace{4ex}
	\end{subfigure}%% 
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/38} 
		\vspace{4ex}
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/39} 
		\vspace{4ex}
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/40}
		\vspace{4ex} 
	\end{subfigure}%%
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/41} 
		\vspace{4ex}
	\end{subfigure}%% 
	\begin{subfigure}[b]{0.09\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figures/gtsrb/42} 
		\vspace{4ex}
	\end{subfigure}%%
	\caption[GTSRB Datensatz]{Examples images of the GTSRB dataset. Each image represents one class.}
	\label{fig:gtsrb}
\end{figure}


==> method.tex <==
\section{Methods}
In this paper we pose the supervised learning problem in terms of a probability distribution $p(\class|\data; \theta )$, where $\class$ denotes the class, $\data$ denotes the input data or image and finally $\theta$ is the parameter vector of the network. In explainable models we are interested in jointly learning the distribution of the output class and the explaining variables $\attri$; we call these variables attributes.
The joint probability distribution of a the class and attributes given input data can be written as 
\begin{equation}
p(\class, \attri|\data; \theta).
\end{equation}

Due to the fact we are using a one-hot encoded description of class-labels and attributes for the $\idxdata$th data sample $\data^{(\idxdata)}$, we can model the conditional probability distribution as a mixture of two categorical distributions 
\begin{equation}
p(\class^{(\idxdata)},\attri^{(\idxdata)}|\data^{(\idxdata)}; \theta)  = \prod_{\idxa = 1}^{\numclasses} \left( \hat{\class}^{(\idxdata)}_\idxa \right)^{\class^{(\idxdata)}_\idxa} \cdot \prod_{\idxb = 1}^{\numattri} \left( \hat{\attri}^{(\idxdata)}_\idxb \right)^{\attri^{(\idxdata)}_\idxb},
\end{equation}
where $\numclasses$ denotes the number of classes and $\numattri$ the number of attributes, respectively. Furthermore, we use the softmax outputs $\hat{\class}\left(\data^{(\idxdata)}; \theta\right)$ and $\hat{\attri}\left(\data^{(\idxdata)}; \theta\right)$ of the network, or in abbreviated form $\hat{\class}^{(\idxdata)}$ and $ \hat{\attri}^{(\idxdata)}$. (ist eigentlich noch falsch, da die Abhängigkeiten fehlen, d.h. z.B. $\hat{\class}\left(\data^{(\idxdata)}, \hat{\attri}^{(\idxdata)}\right)$)

In general the parameter vector $\theta$ is determined using maximum likelihood estimation. The resulting cross-entropy loss between the empirical data distribution $\hat{p}_{data}$ and the model distribution $p$ is given by
\begin{equation}
	L(\theta)= -\mathbb{E}_{\class, \attri, \data \sim \hat{p}_{data}} \log p(\class, \attri|\data; \theta).
\end{equation}
Using our categorical distribution $p (\class, \attri|\data; \theta)$ and a dirac delta distribution for the empirical data we obtain the following loss function 
\begin{equation}
L(\theta)  = - \sum_{\idxa = 1}^{\numclasses} \sum_{i = 1}^\numdata \class_\idxa^{(\idxdata)} \log \hat{\class}_\idxa^{(\idxdata)} - \sum_{\idxb = 1}^{\numattri}  \sum_{\idxdata = 1}^\numdata \attri_\idxb^{(\idxdata)} \log \hat{\attri}_\idxb^{(\idxdata)},
\end{equation}
where $\numdata$ is the total number of training samples. (Vielleicht lassen wir das weg, da hier auch die Abhängigkeiten nicht klar raus kommen). 

The decomposition that is proposed in the following sections can be applied to and/or combined with methods like LIME \cite{Ribeiro2016}. The main difference is that attribution of image regions $R$ are combined in an unsupervised fashion to construct an explanation $\attri$. In order to obtain interpretable image regions the  loss-function can be enriched with a regularization term by using a maximum a posteriori (MAP) estimate. The resulting loss-function is given by 
\begin{align*}
L(\theta)  =& -\mathbb{E}_{\class, \attri, \data, \theta \sim \hat{p}}  \log  p(\theta | \attri, \class, \data, R)\\
=&-\mathbb{E}_{\class, \attri, \data, \theta \sim \hat{p}} \left[  \log p (\class,\attri| \data,\theta, R) + \log p(\theta)  \right],
\end{align*}
where $\hat{p}$ includes the empirical data distribution and the prior distribution over the parameters of the explaining model. 
\subsection{Explanation Dependency Decomposition (EDD)}
This section presents the details of the proposed method regarding the decomposition of different dependencies between attributes and class-labels. We start with a reference model, where no explaining variables are included. Based on this reference, the dependencies are integrated into the probabilistic model and the assumptions as well as the implications are discussed. 

In the following sections it is necessary to distinguish between parameters of the feature extractor $\theta_{f}$ (convolutional layers), classifier $\theta_{\class}$ and explanation or attributes $\theta_{\attri}$, respectively. Up to now we have used the parameter vector $\theta$ to denote all model parameters, that is $\theta=(\theta_{\class},\; \theta_{\attri},\; \theta_{f})$.    

\begin{figure*}
	\centering
	\begin{subfigure}[c]{0.3\textwidth}
		\centering
		\includegraphics[scale=.7]{figures/md}
		\caption{Model: \mref}
		\label{fig:mref}
	\end{subfigure}
	\begin{subfigure}[c]{0.3\textwidth}
		\centering
		\includegraphics[scale=.7]{figures/mc}
		\caption{Model \mfi}
		\label{fig:mfi}
	\end{subfigure}
	\begin{subfigure}[c]{0.3\textwidth}
		\centering
		\includegraphics[scale=.7]{figures/mb}
		\caption{Model \miacd}
		\label{fig:miacd}
	\end{subfigure}
	\begin{subfigure}[c]{0.3\textwidth}
		\centering
		\includegraphics[scale=.7]{figures/ma}
		\caption{Model \mdacd}
		\label{fig:mdacd}
	\end{subfigure}%
	\begin{subfigure}[c]{0.3\textwidth}
		\centering
		\includegraphics[scale=.7]{figures/mf}
		\caption{Model \mcdia}
		\label{fig:mcdia}
	\end{subfigure}
	\begin{subfigure}[c]{0.3\textwidth}
		\centering
		\includegraphics[scale=.7]{figures/me}
		\caption{Model \mcdda}
		\label{fig:mcdda}
	\end{subfigure}
	\caption{Overview of the used models.}
	\label{fig:models}
\end{figure*}

\subsubsection{Reference Model (\mref)}

The first model is a standard classification model, without any explaining variables. This model is used as reference to verify the proposition of \cite{Turner2015} that additional attributes used for explanation may limit the learning freedom of the network and thus lead to worse results. The probability distribution of this network can therefore be written as $p(\class |\data; \theta)$, with $\theta=(\theta_{\class}, \theta_{f})$. 
Fig. \ref{fig:mref} shows the schematic representation of the network divided into the input data $\data$, the convolution network, the classifier (fully connected layer), and the class-output $\class$.

\subsubsection{Full Independence (\mfi)} 
The simplest way of integrating explanations is to assume full independence. The assumptions made in this model (\mfi) are that the attributes are independent of each other and in the same way the class is independent of the attributes. The implication of these assumptions are, that, given the input data $\data$ the attributes $\attri$ are not providing any additional information to solve the classification task $\class$ and vice versa. The probabilistic model for defining the loss-function can be factorizes as 
\begin{equation}
\begin{split}
p(\class, \attri |\data; \theta) & = p(\class|\data; \theta) p(\attri|\class,\data; \theta)\\
& = p(\class|\data; \theta) p(\attri|\data; \theta)\\
& = p(\class|\data; \theta_{\class,f}) \prod_{\idxb = 1}^{\numattri} p(\attri_{\idxb}|\data; \theta_{\attri,f}).
\end{split}
\label{equ:mfi}
\end{equation}
It is assumed, that during the joint training process the attributes and classes can have an influence on the parameter adjustment of feature extractor $\theta_f$. In contrast, the parameters of the model that are dedicated to the attributes $\theta_{\attri}$ are not adjusted by the classification loss and vise versa. 
The corresponding network structure is visualized in Fig. \ref{fig:mfi}.


\subsubsection{Independent Attributes with a Class-Dependency (\miacd)}

When designing an explainable model we want to get an explanation for a specific decision of the model. In this case the assumption that the explaining attributes are independent of the class may be oversimplified. To incorporate the class information we use the model \miacd, where we only assumed independent attributes
\begin{equation}
\begin{split}
p(\class, \attri |\data; \theta) & = p(\class|\data; \theta) p(\attri|\class,\data; \theta)\\
& = p(\class|\data; \theta_{\class,f}) \prod_{\idxb = 1}^{\numattri} p(\attri_{\idxb}|\class, \data; \theta).
\end{split}
\label{equ:miacd}
\end{equation}
Thus, the explaining part of the model is given the ability to focus on class-specific explanations. 
The joint training process of the class and attributes may be instable, since the attribute model has to use the noisy class outputs. To overcome this problem we apply a teacher forcing using the ground-truth labels during the first iterations of the training process. The network structure is shown in Fig. \ref{fig:miacd} and it is obvious that the explaining part of the model can influence all parameters of network, including the classifier. This aspect is possibly restricting the classification performance.  

\subsubsection{Dependent Attributes with a Class-Dependency (\mdacd)}

Using \miacd \, as a base-model, thus preserving the class-dependency of the attributes, in addition a dependency among each attribute can be considered (cp. Fig. \ref{fig:mdacd}). This model has the minimal amount of assumptions possible as well as the model \mcdda. Therefore, the model can capture e.g. the dependence of shape and color attributes. The decomposed probabilistic model used for the loss is given by    
\begin{equation}
\begin{split}
p(\class, \attri |\data; \theta) =& p(\class|\data; \theta) p(\attri|\class,\data; \theta)\\
 =&p(\class|\data; \theta_{\class,f}) \prod_{\idxb = 1}^{\numattri} p(\attri_{\idxb}|\{\attri_{\idxb+1},\dots , \attri_{\numattri}\},\class, \data; \theta).
\end{split}
\label{equ:mdacd}
\end{equation}

\subsubsection{Class Dependent on Attributes and Independent Attributes}

In the previous sections we have assumed a specific order while decomposing the joint probability distribution $p(\class, \attri |\data; \theta)$ (cp. Eq. \ref{eq:miacd}). The goal was to get a explanation for a specific decision of a classifier. A different way to look at the problem is to give a possible explanation first (what kind of attributes are visible in the input space?) and define a classifier to leverage explanations for an enhanced classification performance. Thus, we still obtain an explainable model with slight shift of the objective with focus on the classification performance.   

\begin{equation}
\begin{split}
p(\class, \attri |\data; \theta) & = p(\attri|\data; \theta) p(\class|\attri,\data; \theta)\\
& = p(\class|\data; \theta) p(\attri|\data; \theta)\\
& = p(\class|\data; \theta_{\class,f}) \prod_{\idxb = 1}^{\numattri} p(\attri_{\idxb}|\data; \theta_{\attri,f}).
\end{split}
\label{equ:mc}
\end{equation}

Model \mcdia
Eigentlich müsste hier auch noch die Abhängigkeit der Attribute untereinander mit rein 


\subsubsection{Class Dependent on Attributes and Dependent Attributes}
Model \mcdda


%Model $M_a$
\subsubsection{Pre-training of a Feature Extractor for Classification}
In this model, the mutual influence of the learning process of the class and the attributes is prevented by initially only training the class. Then the corresponding parameters are "frozen" and the attributes are learned. The architecture is the same as in model \mpc.

\begin{equation}
	p(\class, \attri|\data; \theta) = p(\class|\data; \theta) \int p(\attri|\features; \class; \theta) p(\features|\data; \theta) \text{d}\features
\end{equation}

\subsubsection{Pre-training of a Feature Extractor for Attributes}
As an example \mpf

\begin{equation}
p(\class, \attri|\data; \theta) = p(\attri|\data; \theta) \int p(\class|\features; \attri; \theta) p(\features|\data; \theta) \text{d}\features
\end{equation}


==> modells.tex <==
\section{Models}

Five different models:

\begin{itemize}
	\item default classifing cnn
	\item default cnn with indepenedend attributes
	\item default cnn with depenedend attributes
	\item cnn with independend attributes contributing to the class
	\item cnn with dependend attributes contributing to the class
\end{itemize}

%\begin{figure*}
%	\begin{center}
%		%\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%		\centering
%		\begin{subfigure}[t]{0.24\textwidth}
%			\centering
%			\includegraphics[height=1.2in]{figures/m2.pdf}
%			\caption{Model 2}
%		\end{subfigure}%
%		\begin{subfigure}[t]{0.24\textwidth}
%			\centering
%			\includegraphics[height=1.2in]{figures/m2.pdf}
%			\caption{Model 2}
%		\end{subfigure}%
%		\begin{subfigure}[t]{0.24\textwidth}
%			\centering
%			\includegraphics[height=1.2in]{figures/m3.pdf}
%			\caption{Model 3}
%		\end{subfigure}%
%		\begin{subfigure}[t]{0.24\textwidth}
%			\centering
%			\includegraphics[height=1.2in]{figures/m4.pdf}
%			\caption{Model 4}
%		\end{subfigure}%
%	\end{center}
%	\caption{Example of a short caption, which should be centered.}
%	\label{fig:short}
%\end{figure*}

\begin{figure*}[!ht]
	\centering
	\includegraphics[width=\linewidth]{figures/overview.pdf}
	\caption{Overview of our approach. The input images are processeced through five convolutional layer and three dense layer. At the second convolutional layer the color is classified, while the shape is predicted at the third convolutional layer. The symbols are classified at the fifth layer. The results of these three predictions are then passed to the last dense layer.}
	\label{fig:overview}
\end{figure*}

\begin{figure}[!ht]
	\centering
	\includegraphics{figures/m2.pdf}
	\caption{Model 2.}
	\label{fig:m2}
\end{figure}

\begin{figure}[!ht]
	\centering
	\includegraphics{figures/m3.pdf}
	\caption{Model 3.}
	\label{fig:m3}
\end{figure}

\begin{figure}[!ht]
	\centering
	\includegraphics{figures/m4.pdf}
	\caption{Model 4.}
	\label{fig:m4}
\end{figure}
